Symplectic Mapping Class Group Relations Generalizing the Chain Relation

In this paper, we examine mapping class group relations of some symplectic manifolds. For each $n\geq 1$ and $k \geq 1$, we show that the $2n$-dimensional Weinstein domain $W = \{f=\delta\} \cap B^{2n+2}$, determined by the degree $k$ homogeneous polynomial $f\in \mathbb{C}[z_0,\dots,z_n]$, has a Boothby-Wang type boundary and a right-handed fibered Dehn twist along the boundary that is symplectically isotopic to a product of right-handed Dehn twists along Lagrangian spheres. We also present explicit descriptions of the symplectomorphisms in the case $n=2$ recovering the classical chain relation for the torus with two boundary components.

==> paperbib.tex <==
%% This BibTeX bibliography file was created using BibDesk.
%% http://bibdesk.sourceforge.net/


%% Created for Bahar Acu at 2016-09-06 15:09:38 -0700 


%% Saved with string encoding Unicode (UTF-8) 



@phdthesis{vK2,
	Author = {Otto van Koert},
	Date-Added = {2016-09-06 22:07:54 +0000},
	Date-Modified = {2016-09-06 22:09:38 +0000},
	School = {Universit{\"a}t zu K{\"o}ln},
	Title = {Open books for contact five-manifolds and applications of contact homology},
	Year = {2005}}

@book{AD,
	Author = {Alexandru Dimca},
	Date-Added = {2015-09-16 02:22:50 +0000},
	Date-Modified = {2015-09-16 02:35:27 +0000},
	Publisher = {Springer-Verlag, New York},
	Series = {Universitext},
	Title = {Singularities and topology of hypersurfaces},
	Year = {1992}}

@article{WWW,
	Author = {Weiwei Wu},
	Date-Added = {2015-09-14 02:16:41 +0000},
	Date-Modified = {2015-09-16 00:07:06 +0000},
	Journal = {Mathematische Annalen},
	Number = {1},
	Pages = {153-168},
	Title = {Exact {L}agrangians in ${A}_n$-surface Singularities},
	Volume = {359},
	Year = {2014}}

@article{Mat,
	Author = {Matsumoto, Makoto},
	Date-Added = {2015-07-31 01:10:45 +0000},
	Date-Modified = {2015-07-31 01:12:17 +0000},
	Journal = {Mathematische Annalen},
	Number = {3},
	Pages = {401-418},
	Title = {A presentation of mapping class groups in terms of {A}rtin groups and geometric monodromy of singularities},
	Volume = {316},
	Year = {2000}}

@article{PS,
	Author = {P. Seidel},
	Date-Added = {2015-07-12 19:06:26 +0000},
	Date-Modified = {2015-09-16 00:28:34 +0000},
	Journal = {Bulletin de la {S}oci{\'e}t{\'e} {M}ath{\'e}matique de {F}rance},
	Number = {1},
	Pages = {103-149},
	Title = {Graded {L}agrangian Submanifolds},
	Volume = {128},
	Year = {2000}}

@misc{OVK,
	Author = {Otto van Koert},
	Date-Added = {2015-01-05 21:12:04 +0000},
	Date-Modified = {2015-01-05 21:15:12 +0000},
	Month = {October},
	Title = {Personal Communication},
	Year = {2014}}

@misc{DM,
	Author = {Dan Margalit},
	Date-Added = {2014-12-14 06:19:29 +0000},
	Date-Modified = {2014-12-14 06:20:18 +0000},
	Month = {November},
	Title = {Personal Communication},
	Year = {2014}}

@book{IS,
	Author = {Igor R. Shafarevich},
	Date-Added = {2014-12-11 02:51:30 +0000},
	Date-Modified = {2014-12-11 02:57:52 +0000},
	Publisher = {Springer-Verlag},
	Title = {Basic Algebraic Geometry 1: Varieties in Projective Space},
	Year = {2013}}

@book{FM,
	Author = {B. Farb and D. Margalit},
	Date-Added = {2014-11-21 01:45:12 -0800},
	Date-Modified = {2014-11-21 01:48:52 -0800},
	Publisher = {Princeton University Press},
	Title = {A Primer on mapping class groups},
	Volume = {49},
	Year = {2012}}

@book{M2,
	Author = {J. Milnor},
	Date-Added = {2014-10-30 22:35:46 -0700},
	Date-Modified = {2014-10-30 22:36:32 -0700},
	Publisher = {Princeton University Press},
	Series = {Annals of Mathematics Studies},
	Title = {Morse Theory},
	Year = {1963}}

@book{M,
	Author = {J. Milnor},
	Date-Added = {2014-10-29 15:47:25 -0700},
	Date-Modified = {2015-09-16 02:48:45 +0000},
	Number = {61},
	Publisher = {Princeton University Press},
	Series = {Annals of Mathematics Studies},
	Title = {Singular Points of Complex Hypersurfaces},
	Year = {1968}}

@article{SG,
	Author = {S. Gervais},
	Date-Added = {2014-10-22 21:20:39 -0700},
	Date-Modified = {2014-10-22 21:22:41 -0700},
	Journal = {American Mathematical Society},
	Month = {August},
	Number = {8},
	Pages = {3097-3132},
	Title = {Presentation and Central Extensions of Mapping Class Groups},
	Volume = {348},
	Year = {1996}}

@book{GS,
	Author = {R. E. Gompf and A. I. Stipsicz},
	Date-Added = {2014-10-20 16:07:25 -0700},
	Date-Modified = {2014-10-24 00:47:52 -0700},
	Editor = {Am. Math. Soc},
	Pages = {558},
	Series = {Graduate Studies in Mathematics},
	Title = {4-Manifolds and {K}irby calculus},
	Volume = {20},
	Year = {1999}}

@article{HKP,
	Author = {S. Harvey and K. Kawamuro and O. Plamenevskaya},
	Date-Added = {2014-10-20 15:38:04 -0700},
	Date-Modified = {2014-10-20 17:06:51 -0700},
	Journal = {Preprint, arXiv:0712.1557},
	Title = {On Transverse Knots and Branched Covers},
	Year = {2007}}

@book{A,
	Author = {V. I. Arnol'd},
	Date-Added = {2014-10-17 22:05:46 -0700},
	Date-Modified = {2014-10-17 22:10:29 -0700},
	Journal = {Floer Memorial Volume},
	Pages = {99-103},
	Publisher = {Birkh{\"a}user Basel},
	Series = {Progr. Math.},
	Title = {Some remarks on symplectic monodromy of {M}ilnor fibrations},
	Volume = {133},
	Year = {1995}}

@article{PST,
	Author = {P. Seidel},
	Date-Added = {2014-10-17 22:02:00 -0700},
	Date-Modified = {2014-10-17 22:03:38 -0700},
	Journal = {Ph.D. Thesis, {O}xford University},
	Title = {Floer homology and the symplectic isotopy problem},
	Year = {1997}}

@article{AW,
	Author = {A. Wand},
	Date-Added = {2014-10-17 21:45:18 -0700},
	Date-Modified = {2014-10-17 21:52:50 -0700},
	Journal = {Preprint, arXiv:1404.1705},
	Title = {Tightness is preserved by {L}egendrian surgery},
	Year = {2014}}

@article{RA,
	Author = {R. Avdek},
	Date-Added = {2014-10-17 21:42:46 -0700},
	Date-Modified = {2014-10-17 21:51:44 -0700},
	Journal = {Algebraic and Geometric Topology},
	Pages = {1613-1660},
	Title = {Contact Surgery and supporting open books},
	Volume = {13},
	Year = {2013}}

@article{D,
	Author = {S. K. Donaldson},
	Date-Added = {2014-09-26 15:12:08 -0700},
	Date-Modified = {2014-09-26 15:14:43 -0700},
	Journal = {Journal of Differential Geometry},
	Pages = {666-705},
	Title = {Symplectic Submanifolds and almost-complex geometry},
	Volume = {44},
	Year = {1996}}

@article{P2,
	Author = {P. Seidel},
	Date-Added = {2014-09-05 12:33:24 -0700},
	Date-Modified = {2014-09-09 15:43:59 -0700},
	Journal = {Zurich Lectures in Advanced Mathematics, European Mathematical Society (EMS), Vol. VII, Z{\"u}rich},
	Title = {Fukaya categories and {P}icard-{L}efschetz theory},
	Year = {2008}}

@article{KS,
	Author = {M. Khovanov and P. Seidel},
	Date-Added = {2014-08-28 17:24:06 -0700},
	Date-Modified = {2014-09-09 15:44:27 -0700},
	Journal = {Journal of the American Mathematical Society, 15(1)},
	Pages = {203-271 (electronic)},
	Title = {Quivers, {F}loer cohomology and Braid Group Actions},
	Year = {2002}}

@article{G,
	Author = {E. Giroux},
	Date-Added = {2014-08-25 21:51:11 -0700},
	Date-Modified = {2014-09-09 15:44:53 -0700},
	Journal = {Proceedings of the International Congress of Mathematicians, Vol. II},
	Pages = {405-414},
	Title = {G{\'e}ometrie de contact: de la dimension trois vers les dimensions sup{\'e}rieures},
	Year = {Beijing, 2002}}

@article{CDK2,
	Author = {R. Chiang and F. Ding and O. van Koert},
	Date-Added = {2014-07-17 14:39:14 +0300},
	Date-Modified = {2015-01-05 21:31:06 +0000},
	Eprint = {1312.3526},
	Journal = {Preprint, arXiv:1312.3526},
	Title = {Non-fillable invariant contact structures on principal circle bundles and left-handed twists},
	Url = {http://arxiv.org/abs/1312.3526},
	Year = {2013},
	Bdsk-Url-1 = {http://arxiv.org/abs/1312.3526}}

@article{TW,
	Author = {W. P. Thurston and H. E. Winkelnkemper},
	Date-Added = {2014-07-15 21:17:14 +0300},
	Date-Modified = {2014-09-09 15:45:45 -0700},
	Journal = {Proceedings of AMS, Vol. 52},
	Number = {1},
	Pages = {345-347},
	Title = {On the Existence of Contact Forms},
	Year = {1975},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUGJCVYJHZlcnNpb25YJG9iamVjdHNZJGFyY2hpdmVyVCR0b3ASAAGGoKgHCBMUFRYaIVUkbnVsbNMJCgsMDxJXTlMua2V5c1pOUy5vYmplY3RzViRjbGFzc6INDoACgAOiEBGABIAFgAdccmVsYXRpdmVQYXRoWWFsaWFzRGF0YV8QOi4uL1BoRC9SZWZlcmVuY2VzL1RXLU9uIHRoZSBleGlzdGVuY2Ugb2YgY29udGFjdCBmb3Jtcy5wZGbSFwsYGVdOUy5kYXRhTxECBgAAAAACBgACAAAMTWFjaW50b3NoIEhEAAAAAAAAAAAAAAAAAAAAz9PIVkgrAAAACe1kH1RXLU9uIHRoZSBleGlzdGVuY2UgbyNBOUFERS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAKmt7P6sBcUERGIENBUk8AAQADAAAJIAAAAAAAAAAAAAAAAAAAAApSZWZlcmVuY2VzABAACAAAz9QqxgAAABEACAAAz+sizAAAAAEAFAAJ7WQACeooAAnfoAAJ3zoAAmb5AAIAV01hY2ludG9zaCBIRDpVc2VyczoAYmFoYXJhY3U6AERlc2t0b3A6AFBoRDoAUmVmZXJlbmNlczoAVFctT24gdGhlIGV4aXN0ZW5jZSBvI0E5QURFLnBkZgAADgBSACgAVABXAC0ATwBuACAAdABoAGUAIABlAHgAaQBzAHQAZQBuAGMAZQAgAG8AZgAgAGMAbwBuAHQAYQBjAHQAIABmAG8AcgBtAHMALgBwAGQAZgAPABoADABNAGEAYwBpAG4AdABvAHMAaAAgAEgARAASAE5Vc2Vycy9iYWhhcmFjdS9EZXNrdG9wL1BoRC9SZWZlcmVuY2VzL1RXLU9uIHRoZSBleGlzdGVuY2Ugb2YgY29udGFjdCBmb3Jtcy5wZGYAEwABLwAAFQACAA///wAAgAbSGxwdHlokY2xhc3NuYW1lWCRjbGFzc2VzXU5TTXV0YWJsZURhdGGjHR8gVk5TRGF0YVhOU09iamVjdNIbHCIjXE5TRGljdGlvbmFyeaIiIF8QD05TS2V5ZWRBcmNoaXZlctEmJ1Ryb290gAEACAARABoAIwAtADIANwBAAEYATQBVAGAAZwBqAGwAbgBxAHMAdQB3AIQAjgDLANAA2ALiAuQC6QL0Av0DCwMPAxYDHwMkAzEDNANGA0kDTgAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAANQ}}

@article{BW,
	Author = {W. M. Boothby and H. C. Wang},
	Date-Added = {2014-07-15 21:10:25 +0300},
	Date-Modified = {2014-09-09 15:45:20 -0700},
	Journal = {Annals of Math, Vol. 68},
	Number = {3},
	Pages = {721-734},
	Title = {On Contact Manifolds},
	Year = {1958},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUGJCVYJHZlcnNpb25YJG9iamVjdHNZJGFyY2hpdmVyVCR0b3ASAAGGoKgHCBMUFRYaIVUkbnVsbNMJCgsMDxJXTlMua2V5c1pOUy5vYmplY3RzViRjbGFzc6INDoACgAOiEBGABIAFgAdccmVsYXRpdmVQYXRoWWFsaWFzRGF0YV8QLS4uL1BoRC9SZWZlcmVuY2VzL0JXLU9uIENvbnRhY3QgTWFuaWZvbGRzLnBkZtIXCxgZV05TLmRhdGFPEQHcAAAAAAHcAAIAAAxNYWNpbnRvc2ggSEQAAAAAAAAAAAAAAAAAAADP08hWSCsAAAAJ7WQbQlctT24gQ29udGFjdCBNYW5pZm9sZHMucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAqa1M/qvaFQREYgQ0FSTwABAAMAAAkgAAAAAAAAAAAAAAAAAAAAClJlZmVyZW5jZXMAEAAIAADP1CrGAAAAEQAIAADP6yARAAAAAQAUAAntZAAJ6igACd+gAAnfOgACZvkAAgBTTWFjaW50b3NoIEhEOlVzZXJzOgBiYWhhcmFjdToARGVza3RvcDoAUGhEOgBSZWZlcmVuY2VzOgBCVy1PbiBDb250YWN0IE1hbmlmb2xkcy5wZGYAAA4AOAAbAEIAVwAtAE8AbgAgAEMAbwBuAHQAYQBjAHQAIABNAGEAbgBpAGYAbwBsAGQAcwAuAHAAZABmAA8AGgAMAE0AYQBjAGkAbgB0AG8AcwBoACAASABEABIAQVVzZXJzL2JhaGFyYWN1L0Rlc2t0b3AvUGhEL1JlZmVyZW5jZXMvQlctT24gQ29udGFjdCBNYW5pZm9sZHMucGRmAAATAAEvAAAVAAIAD///AACABtIbHB0eWiRjbGFzc25hbWVYJGNsYXNzZXNdTlNNdXRhYmxlRGF0YaMdHyBWTlNEYXRhWE5TT2JqZWN00hscIiNcTlNEaWN0aW9uYXJ5oiIgXxAPTlNLZXllZEFyY2hpdmVy0SYnVHJvb3SAAQAIABEAGgAjAC0AMgA3AEAARgBNAFUAYABnAGoAbABuAHEAcwB1AHcAhACOAL4AwwDLAqsCrQKyAr0CxgLUAtgC3wLoAu0C+gL9Aw8DEgMXAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAxk=}}

@article{BiG,
	Author = {P. Biran and E. Giroux},
	Date-Added = {2014-07-15 21:03:54 +0300},
	Date-Modified = {2014-09-09 15:47:07 -0700},
	Journal = {unpublished manuscript 2005-6, slides of a talk},
	Title = {Symplectic mapping classes and fillings},
	Year = {2007}}

@article{P,
	Author = {P. Seidel},
	Date-Added = {2014-07-15 21:02:33 +0300},
	Date-Modified = {2014-09-09 15:46:37 -0700},
	Eprint = {math/9803084},
	Journal = {Preprint, arXiv:9803084},
	Title = {Symplectic automorphisms of cotangent bundle of sphere},
	Url = {http://arxiv.org/abs/math/9803084},
	Year = {1998},
	Bdsk-Url-1 = {http://arxiv.org/abs/math/9803084}}

@article{CDK,
	Author = {R. Chiang and F. Ding and O. van Koert},
	Date-Added = {2014-07-15 20:59:19 +0300},
	Date-Modified = {2015-01-05 21:30:39 +0000},
	Eprint = {1211.0201},
	Journal = {Preprint, arXiv:1211.0201},
	Title = {Open books for {B}oothby-{W}ang bundles, fibered {D}ehn twists and the mean {E}uler characteristic},
	Url = {http://arxiv.org/abs/1211.0201},
	Year = {2012},
	Bdsk-Url-1 = {http://arxiv.org/abs/1211.0201}}

